Understanding Users' Dissatisfaction with ChatGPT Responses: Types, Resolving Tactics, and the Effect of Knowledge Level

Large language models (LLMs) with chat-based capabilities, such as ChatGPT, are widely used in various workflows. However, due to a limited understanding of these large-scale models, users struggle to use this technology and experience different kinds of dissatisfaction. Researchers have introduced several methods, such as prompt engineering, to improve model responses. However, they focus on enhancing the model's performance in specific tasks, and little has been investigated on how to deal with the user dissatisfaction resulting from the model's responses. Therefore, with ChatGPT as the case study, we examine users' dissatisfaction along with their strategies to address the dissatisfaction. After organizing users' dissatisfaction with LLM into seven categories based on a literature review, we collected 511 instances of dissatisfactory ChatGPT responses from 107 users and their detailed recollections of dissatisfactory experiences, which we released as a publicly accessible dataset. Our analysis reveals that users most frequently experience dissatisfaction when ChatGPT fails to grasp their intentions, while they rate the severity of dissatisfaction related to accuracy the highest. We also identified four tactics users employ to address their dissatisfaction and their effectiveness. We found that users often do not use any tactics to address their dissatisfaction, and even when using tactics, 72% of dissatisfaction remained unresolved. Moreover, we found that users with low knowledge of LLMs tend to face more dissatisfaction on accuracy while they often put minimal effort in addressing dissatisfaction. Based on these findings, we propose design implications for minimizing user dissatisfaction and enhancing the usability of chat-based LLM.

==> tables/dataset_description.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
% \usepackage{longtable}
% Note: It may be necessary to compile the document several times to get a multi-page table to line up properly
\begin{small}
\begin{longtable}[t!]{llll|p{0.06\textwidth}|p{0.40\textwidth}|p{0.15\textwidth}}
\toprule
\multicolumn{4}{l|}{\textbf{Field}} &
  \multicolumn{1}{p{0.06\textwidth}|}{\textbf{Type}} &
  \multicolumn{1}{p{0.40\textwidth}|}{\textbf{Description}} &
  \multicolumn{1}{p{0.20\textwidth}}{\textbf{Example}} \\ \hline
\midrule

\endfirsthead % header
\toprule
\multicolumn{4}{l|}{\textbf{Field}} &
  \multicolumn{1}{p{0.06\textwidth}|}{\textbf{Type}} &
  \multicolumn{1}{p{0.40\textwidth}|}{\textbf{Description}} &
  \multicolumn{1}{p{0.20\textwidth}}{\textbf{Example}} \\ 
\midrule
\endhead

\multicolumn{4}{l|}{\textbf{user\_id}} &
  string &
  Unique identifier for a user &
  cCbpmERyodVxu \\ \hline
\multicolumn{4}{l|}{\textbf{user\_info}} &
  Object &
  Nested structure containing the information about the user &
   \\ \hline
\multicolumn{1}{l|}{} &
  \multicolumn{3}{l|}{\textbf{age}} &
  number &
  User's age &
  23 \\ \hline
\multicolumn{1}{l|}{} &
  \multicolumn{3}{l|}{\textbf{gender}} &
  string &
  User's gender &
  female \\ \hline
\multicolumn{1}{l|}{} &
  \multicolumn{3}{l|}{\textbf{job}} &
  string &
  User's job &
  Engineer \\ \hline
\multicolumn{1}{l|}{} &
  \multicolumn{3}{l|}{\textbf{first\_language}} &
  string &
  User's first language &
  English \\ \hline
\multicolumn{1}{l|}{} &
  \multicolumn{3}{l|}{\textbf{LLM\_knowledge}} &
  Object &
   &
   \\ \hline
 &
  \multicolumn{1}{l|}{} &
  \multicolumn{2}{l|}{\textbf{knowledge\_level}} &
  ordinal number &
  User's knowledge level regarding LLM on a 7-point scale (1: very low, 7: very high) &
  6 \\ \hline
 &
  \multicolumn{1}{l|}{} &
  \multicolumn{2}{l|}{\textbf{knowledge\_level\_reason}} &
  string &
  The reason for user's knowledge level &
  I have been studying LLM for 3 years. \\ \hline
\multicolumn{1}{l|}{} &
  \multicolumn{3}{l|}{\textbf{chatgpt\_general\_experiences}} &
  Object &
  Nested structure containing various fields related to the user's overall experiences with using ChatGPT. &
   \\ \hline
\multicolumn{1}{l|}{} &
  \multicolumn{3}{l|}{\textbf{chatgpt\_usage\_language}} &
  Object &
  Sub-structure containing information about the user's commonly used language with ChatGPT. &
   \\ \hline
 &
  \multicolumn{1}{l|}{} &
  \multicolumn{2}{l|}{\textbf{usage\_language}} &
  string &
  User's commonly used language for interacting with ChatGPT. &
  English \\ \hline
 &
  \multicolumn{1}{l|}{} &
  \multicolumn{2}{l|}{\textbf{writing\_level}} &
  ordinal number &
  User's writing proficiency level about the language on a 7-point scale (1: very low, 7: very high) &
  7 \\ \hline
 &
  \multicolumn{1}{l|}{} &
  \multicolumn{2}{l|}{\textbf{reading\_level}} &
  ordinal number &
  User's reading comprehension level about the language on a 7-point scale (1: very low, 7: very high) &
  6 \\ \hline
\multicolumn{1}{l|}{} &
  \multicolumn{3}{l|}{\textbf{chatgpt\_usage\_purpose}} &
  string &
  The primary purpose or use case of ChatGPT for the user. &
  I used it to get some useful information, summarisation, translation, etc. \\ \hline
\multicolumn{1}{l|}{} &
  \multicolumn{3}{l|}{\textbf{chatgpt\_usage\_period}} &
  string &
  The duration of the user's usage of ChatGPT. &
  1 month \\ \hline
\multicolumn{1}{l|}{} &
  \multicolumn{3}{l|}{\textbf{chatgpt\_usage\_frequency}} &
  string &
  The frequency of the user's usage of ChatGPT. &
  1 time a week \\ \hline
\multicolumn{1}{l|}{} &
  \multicolumn{3}{l|}{\textbf{chatgpt\_overall\_satisfaction}} &
  Object &
  Nested structure containing the user's overall satisfaction with ChatGPT &
   \\ \hline
 &
  \multicolumn{1}{l|}{} &
  \multicolumn{2}{l|}{\textbf{satisfaction\_level}} &
  ordinal number &
  User's overall satisfaction level with ChatGPT on a 7-point scale (1: very low, 7: very high) &
  5 \\ \hline
 &
  \multicolumn{1}{l|}{} &
  \multicolumn{2}{l|}{\textbf{satisfaction\_level\_reason}} &
  string &
  The reason for the user's satisfaction level. &
  I am satisfied with ChatGPT because it is very useful. \\ \hline
\multicolumn{4}{l|}{\textbf{chat\_data\_n}} &
  Object &
  Nested structure that contains detailed information about a specific chat session with ChatGPT. n could be 1 $\sim$5. &
   \\ \hline
\multicolumn{1}{l|}{} &
  \multicolumn{3}{l|}{\textbf{chat\_date}} &
  string &
  Date of that chat session. &
  One week ago \\ \hline
\multicolumn{1}{l|}{} &
  \multicolumn{3}{l|}{\textbf{memory\_level}} &
  ordinal number &
  User's memory level of that chat session on a 7-point scale (1: very poor, 7: Excellent) &
  7 \\ \hline
\multicolumn{1}{l|}{} &
  \multicolumn{3}{l|}{\textbf{model\_version}} &
  string &
  The version of ChatGPT model used in that chat session (gpt3.5 or gpt4). &
  gpt3.5 \\ \hline
\multicolumn{1}{l|}{} &
  \multicolumn{3}{l|}{\textbf{chat\_usage\_language}} &
  string &
  The language used in that chat session. &
  English \\ \hline
\multicolumn{1}{l|}{} &
  \multicolumn{3}{l|}{\textbf{chat\_usage\_language\_reason}} &
  string &
  The reason for using that language in that chat session. &
  because this is my first language \\ \hline
\multicolumn{1}{l|}{} &
  \multicolumn{3}{l|}{\textbf{chat\_purpose}} &
  string &
  The specific purose of that chat session. &
  I want to get some summarise of the article \\ \hline
\multicolumn{1}{l|}{} &
  \multicolumn{3}{l|}{\textbf{why\_chatgpt}} &
  string &
  The motivation or reason for using ChatGPT for that purpose. &
  I thought it is good at summarising \\ \hline
\multicolumn{1}{l|}{} &
  \multicolumn{3}{l|}{\textbf{dissatisfaction\_responses}} &
  Array &
  List of user's experience data related to their dissatisfaction with responses generated by ChatGPT. Each element in the list contains data on each dissatisfactory ChatGPT response. &
   \\ \hline
 &
  \multicolumn{1}{l|}{} &
  \multicolumn{2}{l|}{\textbf{dissatisfaction\_chatgpt\_response}} &
  string &
  ChatGPT response that the user selected as dissatisfactory. &
  Of course, the best books of the year are subjective, but I think the best ... \\ \hline
 &
  \multicolumn{1}{l|}{} &
  \multicolumn{2}{l|}{\textbf{dissatisfaction\_chat\_num}} &
  number &
  The chat turn number of dissatisfaction\_chatgpt\_response among ChatGPT responses.  It starts with 0. &
  2 \\ \hline
 &
  \multicolumn{1}{l|}{} &
  \multicolumn{2}{l|}{\textbf{dissatisfaction\_category\_score}} &
  Object &
  \makecell[l]{Nested structure containing dissatisfaction scores for \\ 
                seven dissatisfaction categories. \\ 
                The dissatisfaction score is an integer value ranging\\ 
                 from 0 to 10. \\
                - 0: No dissatisfaction \\
                - 1: A little dissatisfied \\
                - 10: Extremely dissatisfied} &
   \\ \hline
 &
   &
  \multicolumn{1}{l|}{} &
  \textbf{D\_intent} &
  number &
  Dissatisfaction score in the aspect of "Intent understanding (D\_intent)". &
  2 \\ \hline
 &
   &
  \multicolumn{1}{l|}{} &
  \textbf{D\_depth} &
  number &
  Dissatisfaction score in the aspect of "Content depth and originality (D\_depth)". &
  0 \\ \hline
 &
   &
  \multicolumn{1}{l|}{} &
  \textbf{D\_accuracy} &
  number &
  Dissatisfaction score in the aspect of "Information accuracy (D\_acc)". &
  7 \\ \hline
 &
   &
  \multicolumn{1}{l|}{} &
  \textbf{D\_transparency} &
  number &
  Dissatisfaction score in the aspect of "Transparency (D\_trans)". &
  0 \\ \hline
 &
   &
  \multicolumn{1}{l|}{} &
  \textbf{D\_refuse} &
  number &
  Dissatisfaction score in the aspect of "Refusal to answer (D\_refuse)". &
  0 \\ \hline
 &
   &
  \multicolumn{1}{l|}{} &
  \textbf{D\_ethic} &
  number &
  Dissatisfaction score in the aspect of "Content ethichs and integrity (D\_ethic)". &
  0 \\ \hline
 &
   &
  \multicolumn{1}{l|}{} &
  \textbf{D\_format} &
  number &
  Dissatisfaction score in the aspect of "Response format and attitude (D\_format)". &
  3 \\ \hline
 &
  \multicolumn{1}{l|}{} &
  \multicolumn{2}{l|}{\textbf{dissatisfaction\_overall\_score}} &
  number &
  \makecell[l]{Overall dissatisfaction score of\\ 
                dissatisfaction\_chatgpt\_response ranging from \\ 
                1 to 10. \\ 
                - 1: A little dissatisfied \\ 
                - 10: Extremely dissatisfied} &
  6 \\ \hline
 &
  \multicolumn{1}{l|}{} &
  \multicolumn{2}{l|}{\textbf{dissatisfaction\_reason}} &
  string &
  The reason for the user's dissatisfaction &
  I think the summarisation is not accurate \\ \hline
 &
  \multicolumn{1}{l|}{} &
  \multicolumn{2}{l|}{\textbf{tactics}} &
  Array &
  List of user's tactics employed to address the dissatisfaction. &
   \\ \hline
 &
   &
  \multicolumn{1}{l|}{} &
  \textbf{tactic\_type} &
  string &
  The type of tactic used among `user\_prompt`, `no\_tactic`, `end\_conversation`. &
  user\_prompt \\ \hline
 &
   &
  \multicolumn{1}{l|}{} &
  \textbf{tactic\_prompt} &
  string &
  \makecell[l]{(Optional) \\ 
                When tactic\_type is `user\_prompt`, user's prompt\\
                associated with the tactic. \\ 
                When tactic\_type is `no\_tactic`, empty.\\ 
                When tactic\_type is `end\_conversation`, user's last \\ 
                prompt before terminating the conversation.} &
  Please give me more accurate summarisation \\ \hline
 &
   &
  \multicolumn{1}{l|}{} &
  \textbf{tactic\_prompt\_chat\_num} &
  number &
  \makecell[l]{(Optional) \\ 
                When tactic\_type is `user\_prompt`, the chat turn\\
                number of tactic\_prompt among user's prompt.\\ 
                It starts with 0.} &
  3 \\ \hline
 &
   &
  \multicolumn{1}{l|}{} &
  \textbf{tactic\_effectiveness\_score} &
  number &
  The effectiveness score of the tactic. &
  8 \\ \hline
 &
   &
  \multicolumn{1}{l|}{} &
  \textbf{tactic\_effectiveness\_reason} &
  string &
  The reason for the tactic's effectiveness. &
  I think the answer is more accurate than before. \\ \hline
 &
   &
  \multicolumn{1}{l|}{} &
  \textbf{tactic\_theme} &
  string &
  Thematic category of the tactic among T\_repeat, T\_specify, T\_error, T\_adapt, or No\_tactic. &
  T\_specify \\ \hline
 &
   &
  \multicolumn{1}{l|}{} &
  \textbf{tactic\_code} &
  string &
  Corresponding tactic codes among T\_1 $\sim$T\_13. &
  T4 \\ \hline
\multicolumn{1}{l|}{} &
  \multicolumn{3}{l|}{\textbf{chat\_shared\_link}} &
  string &
  The shared link (URL) of the chat session. It could not be accessed if the user deletes the conversation. &
  https://chat.openai. com/share/aaaaa-aaaaa \\ \hline
\multicolumn{1}{l|}{} &
  \multicolumn{3}{l|}{\textbf{chat\_log}} &
  Arrary &
  List of all chat log entries for the chat session. &
   \\ \hline
 &
  \multicolumn{1}{l|}{} &
  \multicolumn{2}{l|}{\textbf{role}} &
  string &
  `user` or `assistant`. When role is `user`, the contents is user's prompt. When role is `assistant`, the content is response generated by ChatGPT. &
  user \\ \hline
 &
  \multicolumn{1}{l|}{} &
  \multicolumn{2}{l|}{\textbf{content}} &
  string &
  User's prompt or ChatGPT response. &
  Give me a summarisation of this article. Article title:... \\ \hline
\multicolumn{4}{l|}{\textbf{created\_at}} &
  string &
  The timestamp indicates the exact time when the data was created after receiving the user's response. &
  09/04/2023, 15:07:05 \\ 
\bottomrule

\caption{Detailed description of each field of our dataset, including type and example. Note that the indentations in the \textbf{Field} column represent the hierarchical structure of our dataset.}
\label{tab:dataset}\\
\end{longtable}
\end{small}


==> tables/know_tactic.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{cc|cccccccc}
\toprule
\multirow{4}{*}{\makecell[c]{Tactic \\ Category}} &
  \multirow{4}{*}{\makecell[c]{Tactic \\ Code}} &
  \multicolumn{8}{c}{Response-level analysis} & \cline{3-10} 
 &
   &
  \multicolumn{4}{c|}{Count: N (\%)} &
  \multicolumn{4}{c}{Effectiveness Score: mean (std)} \\ \cline{3-10}
 &
   &
  \multicolumn{2}{c}{\textbf{Category*}} &
  \multicolumn{2}{c}{Code} &
  \multicolumn{2}{c}{Category} &
  \multicolumn{2}{c}{Code} & \cline{3-10}
  &
   &
  high &
  low &
  high &
  \multicolumn{1}{c|}{low} &
  high &
  low &
  high &
  low  \\ \hline
\midrule
\multirow{3}{*}{\Trepeat{}} &
  T1 &
  \multirow{3}{*}{16 (6.11\%)} &
  \multirow{3}{*}{\textbf{19 (14.5\%)}} &
  12 (4.4\%) &
  \multicolumn{1}{c|}{9 (6.5\%)} &
  \multirow{3}{*}{\textbf{5.06 (3.00)*}} &
  \multirow{3}{*}{\textbf{2.37 (2.27)*}} &
  4.75 (2.96) &
  3.00 (3.00) & \\
 &
  T2 &
   &
   &
  4 (1.5\%) &
  \multicolumn{1}{c|}{12 (8.7\%)} &
   &
   &
  6.00 (3.37) &
  1.67 (1.15) &
   &
   &
   \\
 &
  T3 &
   &
   &
  1 (0.4\%) &
  \multicolumn{1}{c|}{0 (0.0\%)} &
   &
   &
  1 (-) &
  - (-) &
   &
   &
  0.00 (0.02) &
  0.23 (0.35) \\ \hline
\multirow{4}{*}{\Tspecify{}} &
  T4 &
  \multirow{4}{*}{111 (42.37\%)} &
  \multirow{4}{*}{52 (39.7\%)} & 
  84 (30.8\%) &
  \multicolumn{1}{c|}{24 (17.4\%)} &
  \multirow{4}{*}{5.88 (3.56)} &
  \multirow{4}{*}{6 (3.33)} &
  5.77 (3.71) &
  7.17 (2.78) & \\
 &
  T5 &
   &
   &
  13 (4.8\%) &
  \multicolumn{1}{c|}{12 (8.7\%)} &
   &
   &
  5.00 (3.03) &
  5.42 (3.73) &
   &
   & \\
 &
  T6 &
   &
   &
  19 (7.0\%) &
  \multicolumn{1}{c|}{13 (9.4\%)} &
   &
   &
  7.00 (2.83) &
  6.00 (3.70) &
   &
   & \\
 &
  T7 &
   &
   &
  4 (1.5\%) &
  \multicolumn{1}{c|}{7 (5.1\%)} &
   &
   &
  6.00 (4.08) &
  4.00 (2.31) &
   &
   & \\ \hline
\multirow{3}{*}{\Terror{}} &
  T8 &
  \multirow{3}{*}{\textbf{49 (18.70\%)}} &
  \multirow{3}{*}{8 (6.1\%)} &
  37 (13.6\%) &
  \multicolumn{1}{c|}{5 (3.6\%)} &
  \multirow{3}{*}{3.53 (2.60)} &
  \multirow{3}{*}{5.75 (3.06)} &
  3.81 (4.08) &
  5.2 (3.83) & \\
 &
  T9 &
   &
   &
  7 (2.6\%) &
  \multicolumn{1}{c|}{2.00 (1.4\%)} &
   &
   &
  3.57 (1.90) &
  7.00 (1.41) &
   &
   & \\
 &
  T10 &
   &
   &
  6 (2.2\%) &
  \multicolumn{1}{c|}{2 (1.4\%)} &
   &
   &
  2 (2.45) &
  7.00 (1.41) &
   &
   & \\ \hline
\multirow{3}{*}{\Tadapt{}} &
  T11 &
  \multirow{3}{*}{5 (1.91\%)} &
  \multirow{3}{*}{1 (0.8\%)} &
  4 (1.5\%) &
  \multicolumn{1}{c|}{1 (0.7\%)} &
  \multirow{3}{*}{4.40 (3.29)} &
  \multirow{3}{*}{1 (-)} &
  5.25 (3.10) &
  1 (-) & \\
 &
  T12 &
   &
   &
  0 (0.0\%) &
  \multicolumn{1}{c|}{0 (0.0\%)} &
   &
   &
  - &
  - &
   &
   & \\
 &
  T13 &
   &
   &
  1 (0.4\%) &
  \multicolumn{1}{c|}{0 (0.0\%)} &
   &
   &
  1 (-) &
  - &
   &
   & \\ \hline
\multicolumn{2}{c|}{No Tactic} &
  81 (30.92\%) &
  \textbf{51 (38.9\%)} &
  81 (29.7\%) &
  \multicolumn{1}{c|}{51 (37.0\%)} &
  - &
  - &
  - &
  - & \\
\bottomrule
\end{tabular}%
}
\caption{Tactic category and code for knowledge level high and low group (* p-value \textless 0.01)}
\label{tab:know-tactic}
\end{table*}
